Cosmological constraints from galaxy-lensing cross correlations using BOSS galaxies with SDSS and CMB lensing

We present cosmological parameter constraints based on a joint modeling of galaxy-lensing cross correlations and galaxy clustering measurements in the SDSS, marginalizing over small-scale modeling uncertainties using mock galaxy catalogs, without explicit modeling of galaxy bias. We show that our modeling method is robust to the impact of different choices for how galaxies occupy dark matter halos and to the impact of baryonic physics (at the $\sim2\%$ level in cosmological parameters) and test for the impact of covariance on the likelihood analysis and of the survey window function on the theory computations. Applying our results to the measurements using galaxy samples from BOSS and lensing measurements using shear from SDSS galaxies and CMB lensing from Planck, with conservative scale cuts, we obtain $S_8\equiv\left(\frac{\sigma_8}{0.8228}\right)^{0.8}\left(\frac{\Omega_m}{0.307}\right)^{0.6}=0.85\pm0.05$ (stat.) using LOWZ $\times$ SDSS galaxy lensing, and $S_8=0.91\pm0.1$ (stat.) using combination of LOWZ and CMASS $\times$ Planck CMB lensing. We estimate the systematic uncertainty in the galaxy-galaxy lensing measurements to be $\sim6\%$ (dominated by photometric redshift uncertainties) and in the galaxy-CMB lensing measurements to be $\sim3\%$, from small scale modeling uncertainties including baryonic physics.

==> referee_report <==
>Comments to the Author
>I was asked to report on the paper "Cosmological constraints from
>galaxy-lensing cross correlations using BOSS galaxies with SDSS and
>CMB lensing" by Singh et al. The paper presents a new approach to perform a
>joint analysis of galaxy clustering and galaxy-galaxy lensing
>circumventing an explicit implementation of a bias model to predict
>the galaxy-galaxy  and galaxy-matter correlation function. The basis
>of the approach presented here is that the cross correlation
>coefficient between gg, gm and mm statistics is close to unity and its
>smooth scale dependence can be accounted for by a simple parametric
>model.
>The authors present a careful account of systematics such as
>highly-nonlinear small scale clustering, photometric redshift
>uncertainties and baryonic effects based on a dedicated
>mock/simulation study. They find S8 values significantly lower than
>what is predicted based on the Planck CMB analysis, which is an
>important confirmation of similar tensions reported by other
>low-redshift analyses.
>The novelty of the approach and the rigor in the treatment of
>systematics make this paper well suited for publication in MNRAS. I do
>however have some comments and suggestions for further improvement of
>the paper, which I would kindly ask the authors to consider before
>publication.

We thank the referee for a very positive report and for the comments
that have helped in improving the quality and presentation of the paper. 
We also apologize for the delay in the response.
Our responses are highlighted in cyan in the paper draft.

>Eqs 4-6 are a bit confusing in that they show both \kappa(x) and
>\kappa(k) in the same line with an equal sign. This is mathematically
>incorrect and should be replaced by an alternate notation accounting
>for the the Fourier transform. I also think that there is a minus
>arising in the k-space expressions from \nabla^2\to (i k)^2=-k^2

We have changed the notation and also corrected the sign.

>In Eq. 9 and below, the usage of f_k(\chi) seems a bit excessive and
>confusing, as most of this study seems to be working in the framework
>of a flat Universe.

It is correct that we assume flat universe wherever
necessary. However, we prefer to use the standard (and more general)
notation to denote the transverse comoving distances.

>Eq (11): Introducing a dependence on the transverse separation r_p for
>both the bias and the cross correlation coefficient seems a bit
>excessive, Unless the two functions are defined separately from the
>ratios of gm/mm and gg/mm. But this is not explicitly done in the
>paper. Also, could the authors elaborate what is P_{\delta\delta}(\vec
>k,z)? Does \vec k include the line of sight wavenumber that is being
>integrated over (via z) or is it supposed to be the perpendicular
>wavenumber? Also, the right hand side does not have a \Pi dependence
>but the left hand side (rightfully) implies one. Why are there no
>redshift space distortions for the galaxies in this equation?

We do treat bias and rcc differently in this study, except that we
replace the bias with \sqrt(gg/mm) when writing our model (in section
3). Hence we prefer to keep the discussion general in section 2 and
treat bias and rcc as functions of scale. We have added two new equations
stating bias and rcc explicitly.
We have corrected the discrepancy in equation 11 and added the missing
integral over k_z. There is no RSD in lensing cross correlations as
lensing kernel is broad in redshift and washes out any RSD effects.
Any effects in the lensing kernel from galaxy velocities are superseded 
by much larger photometric redshift errors (from source galaxies).

>Eqs. (12) and (13) are really just one equation so they shouldn't have
>separate equation numbers and a \times would be appropriate in the
>second line. I am a bit confused by the presence and integration over
>z. In my understanding the redshift and the line of sight coordinate
>encode the same information. Also is the weight function W(z) the same
>for Eq 11 and Eq 12/13? I strongly encourage the authors to motivate
>their notation in a bit more detail.

We have corrected the numbering error in the equation and added \times 
(please note that Eq. 12 is Eq. 14 now and the numbering of subsequent 
equation will be different as well.). 
We have also added an explanation of W(z). We distinguish between the 
redshift and line of sight integrations. The line of sight integration 
is done for galaxies at each redshift. Then the contribution from galaxies
at each redshift is added up with the weights W(z). W(z) depends on the
redshift distribution of the galaxies and the explicit and implicit weights 
in the measurement estimator (e.g. in clustering estimator galaxies are
implicitly weighted by the number density). 
W(z) is different for
lensing and clustering and we have changed the notation slightly,
using W_L(z) for the lensing case.
 
>Sec. 2.3.3 Could the authors elaborate why they deem it advantageous
>to first measure the three dimensional correlation function as a
>function of transverse and line-of-sight separation to project
>afterwards. I would have thought that a direct projection of galaxies
>on a transverse plane and calculation of the 2D correlation function
>would have been a more direct approach. Could they motivate the 100
>h^{-1}Mpc integration length? The lensing window is much wider so I
>would suspect a longer line-of-sight integration for the galaxies
>would bring the cross-correlation coefficient closer to unity?

Our code computes the correlation function through direct pair
counting where distances are computed for each pair, accounting for
the spherical geometry. The 100 Mpc/h length is motivated in our
previous papers where these measurements are presented. In short, a
small integration length is desirable to get higher S/N in the
measurements, but a longer integration length is desirable to reduce
the RSD effects. 100 Mpc/h is chosen so that RSD effects are
small on the scales we use. We have added some discussion to the 
section 2.3.3.


>Below Eq. (22) there is a jump in the sentence, basically there seems
>to be a part missing can also be converted"

Corrected. (Eq. 23 now.)

>In Sec. 3, the authors mention emulators, perturbation theory and
>HALOFIT to then mention that the latter is employed. If they are not
>used, mentioning emulators and perturbation theory seems confusing and
>the authors might want to consider to omit them.

We have changed the language.

>Sec. 3: I would encourage the authors to stick to one notation
>regarding r_cc, either r_{cc,\Upsilon} OR r_{cc}^\Upsilon.

Changed. We will use r_{cc}^\Upsilon

>Sec. 3. It would be useful to introduce the modeling notation used
>later in Figures, \Upsilon, \Upsilon \to \Delta\Sigma, \Sigma \to
>\Delta \Sigma

We have added the notation to subsection titles.


>Sec. 3.2.2: Could the authors elaborate what they mean by localized in
>the where r_cc values are more localized in r_p

We have added an explanation.

>Eq (28): the left hand side defines \Sigma_0(r_p), but on the right
>hand side the functional dependence is on r_0.

We have corrected the equation. (please note that it is eq. 29 now)

>In Fig. 1 the caption states that the results would have changed
>insignificantly if r_cc=1 had been assumed throughout. Is this true
>for both \Upsilon and \Sigma? Why is it worth parametrizing r_cc in
>this case?

r_cc=1 is not a correct model. The statement is based on the tests we
discuss in section 5.1.2 to understand the impact of our assumptions
about rcc and that statement is only true within the precision of our
mocks and data and the scales used. Since we know parametric forms fits 
rcc better than rcc fixed to 1, it is worth using the right form. 
One can fix rcc to the value from mocks, but that would imply trusting 
the mocks as true representation of data when we know they are not perfect. 
Hence we do not show the tests with rcc fixed to mocks values and 
instead only show an extreme test with rcc=1.   

>Page 5, right column, first line, there is a full stop in the middle
>of the sentence

Removed.

>Fig 2, In  the caption "using with covariance matrix". It might be worth referencing
>again to the earlier description of priors on r_cc, as it is somewhat
>unusual to put the prior on a function of the parameters (a,b).

This is pointed out in the caption. We have added a reference to section 3.

>Table 2, the caption should mention that these values are for the mock
>study
Done

>Sec. 4.2: it would be good if the authors could define both SHAM and
>HAM abbreviations and stress the difference. As far as I am aware,
>SHAM usually stands for Subhalo Abundance Matching, but is here
>introduced standard Halo Abundance . Also, the section could be
>clearer how exactly the parameters of the HAM model are being tuned to
>match the clustering, i.e., which observed statistics are being
>matched to which simulation statistics.

We have modified the text in Sec. 4.2.


>It is slightly odd that in many of the 2D and 1D posterior triangle
>plots (Figs. 2,7,8a, 9 etc.) the contours are not closed and the 1D
>posteriors are not shown far enough for them to asymptote to the
>x-axis. I think this problem should be rectified in order for the
>reader (and the authors) to be able to assess the full PDF. If these
>points have not been sampled I suggest widening the spread of the
>seeds.
Many of the contours are not closed due to the effects of the priors,
with the priors described in the text. The limits on the plots,
especially in 1d, are decided in an automated way such that at least +/- 3
sigma limits are shown for each curve, where 3 sigma is decided based
on the the full chain. We do not find this to be a limiting factor in
analysis/interpretation of the plots. We have added a line in the caption
explaining the limits on the panels.

>I would urge the authors to try to make sure that font sizes in
>figures are somewhat similar (ideally identical) to the font size used
>in the text. In particular Fig. 9 looks a bit out of proportion.

We have modified the figures 9,11, reducing the text size.

>Figure 3: The upper panel is missing a y-axis label, also, could the
>authors elaborate on the filled contours showing the ratio to the
>Planck cosmology, what determines their height?
Y-axis label is missing because we are plotting two different
quantities and they are labeled in the legend. We have expanded the
description of the filled contours. The height is determined by the
1\sigma errors on S8. We have modified the caption.

>page 13, left column, line 55 small  -> "small scale modeling"
Changed.

>In a perturbative approach to the respective correlation functions,
>the cross-correlation coefficient is a function of the bias
>parameters. Could the authors elaborate on whether the
>cross-correlation coefficients with their fitted parameters are
>mapping to realistic quadratic bias values?

We have not tested this and unfortunately we do not have codes setup to
do so easily. However, given that we get reasonable values of rcc
from mocks and apply a prior based on these, we expect quadratic
bias values to be reasonable.

>Could the authors elaborate which cosmological parameters are fixed
>and which priors are being used in Sec. 5.2

We only vary A_s and Omega_m (with sigma8 being derived from those 
values) and fix all other cosmological parameters. This is 
mentioned it in the beginning of section 5 and we have added text 
in section 5.2 as a reminder for the reader.

>The notation r_{cc,a} and r_{cc,b} in Fig 4 is a bit misleading since
>this hints at these parameters being cross-correlation coefficients
>rather than parameters of the cross-correlation function, maybe a_r
>and b_r would be less confusing?
We understand referee's point, however we believe this is a subjective 
choice and we prefer to stick with our notation as it makes clear that
parameters are related to rcc.

>The abbreviations CL,GL GGL in Fig 9 are not introduced.
Done

>The authors might want to consider equations as part of the sentences
>and include the relevant full stops and comma to make the publication
>more readable.

We have made the changes to the equations.

>Pg 13, left column, line 49: "asssembly" -> "assembly" 
Changed

>In the last paragraph of the conclusion, the authors argue that their
>result of S8 being significantly lower than Planck could be a
>statistical fluctuation. I thought their analysis and error bars
>account for cosmic variance. I would appreciate if they could
>elaborate a bit on this hypothesis.
It is true that our errors account for cosmic variance. The ~3\sigma
tensions, while unlikely, can still possibly be statistical fluctuations. 

